Edit Distance Robust Watermarks via Indexing Pseudorandom Codes

Motivated by the problem of detecting AI-generated text, we consider the problem of watermarking the output of language models with provable guarantees. We aim for watermarks which satisfy: (a) undetectability, a cryptographic notion introduced by Christ, Gunn & Zamir (2024) which stipulates that it is computationally hard to distinguish watermarked language model outputs from the model's actual output distribution; and (b) robustness to channels which introduce a constant fraction of adversarial insertions, substitutions, and deletions to the watermarked text. Earlier schemes could only handle stochastic substitutions and deletions, and thus we are aiming for a more natural and appealing robustness guarantee that holds with respect to edit distance. Our main result is a watermarking scheme which achieves both undetectability and robustness to edits when the alphabet size for the language model is allowed to grow as a polynomial in the security parameter. To derive such a scheme, we follow an approach introduced by Christ & Gunn (2024), which proceeds via first constructing pseudorandom codes satisfying undetectability and robustness properties analogous to those above; our key idea is to handle adversarial insertions and deletions by interpreting the symbols as indices into the codeword, which we call indexing pseudorandom codes. Additionally, our codes rely on weaker computational assumptions than used in previous work. Then we show that there is a generic transformation from such codes over large alphabets to watermarking schemes for arbitrary language models.

==> temp.tex <==
\begin{algorithm}
  \caption{Indexing PRC: $\PRCI[\PRCS, \rho]$}
  \label{alg:prf-di}
  \begin{algorithmic}[1]\onehalfspacing
    \Require PRC for substitutions: $(\KeyS, \EncS, \DecS)$, together with functions $n : \BN \to \BN, \ell : \BN \to \BN$ characterizing the block length and key length, respectively; parameter $\rho > 1$. Functions $m(\lambda) := \lceil \ln(2) \cdot n(\lambda)\rceil $, $\alphb(\lambda):= \rho \cdot n(\lambda)$. 

    \Function{$\Key$}{$1^\lambda$}
    \State Define $\sk \gets \KeyS(1^\lambda)$.
    \State Let $\psi : [\alphb(\lambda)] \to [n(\lambda)]$ be a uniformly random function conditioned on $|\psi^{-1}(j)| = \rho$ for each $j \in [n(\lambda)]$.
    \State \Return $(\sk, \psi)$. 
    \EndFunction

    \Function{$\Enc$}{$1^\lambda, (\sk, \psi), \msg$}
    \State Set $y^0 \gets \EncS(1^\lambda, \sk, \msg) \in \hc[n(\lambda)]$. %
    \State Set $y \gets \PerturbDifference(n(\lambda), m(\lambda), y^0)$.\label{line:pd-call}
    \State For each $j \in [m(\lambda)]$, choose $z_j \sim \Unif( \{ a \ : \ \psi(a) = y_j \})$. \label{line:ybar-sample}
    \State \Return $z = (z_1, \ldots, z_{m(\lambda)})$.

    \EndFunction

    

    \Function{$\Dec$}{$1^\lambda, (\sk, \psi), z$}
    \State Define $y := \psi (z) = (\psi(z_1), \ldots, \psi(z_{m(\lambda)}))$. 
    \State Define $y' \in \hc[n]$ by $y'_i = \One{i \in \Unique(y)}$.\label{line:yprime-decode}
    \State \Return $\DecS(1^\lambda, \sk, y')$. 
    \EndFunction

    
    \Function{$\PerturbDifference$}{$n,m, y^0$}
    \State Set $\MS^0 := \{ i \in [n] \ : \ y^0_i = 1 \}$. \label{line:define-s0}
    \State Sample $y^1 \sim \Unif([n]^m)$.\label{line:sample-y1}
    \State Set $\MS^1 := \Unique(y^1) \subset [n]$.\label{line:define-s1}
    \If{$|\MS^0 \backslash \MS^1| \geq |\MS^1\backslash \MS^0|$}
    \State Let $\sigma : \MS^1 \backslash \MS^0 \to \MS^0 \backslash \MS^1$ denote a uniformly random injective mapping.
    \State For each $a \in \MS^1 \backslash \MS^0$, let $y$ be formed by replacing each instance of $a$ in $y^1$ with $\sigma(a)$.\label{line:replace-sigma}
    \Else
    \State Let $\tau : \MS^0 \backslash \MS^1 \to \MS^1 \backslash \MS^0$ denote a uniformly random injective mapping.
    \State For each $a \in \MS^0 \backslash \MS^1$, let $y$ be formed by replacing each instance of $\tau(a)$ in $y^1$ with $a$. \label{line:replace-tau}
    \EndIf
    \State\Return $y$. 

    \EndFunction
  \end{algorithmic}

\end{algorithm}

==> widebar.tex <==

\makeatletter
\let\save@mathaccent\mathaccent
\newcommand*\if@single[3]{%
  \setbox0\hbox{${\mathaccent"0362{#1}}^H$}%
  \setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}%
  \ifdim\ht0=\ht2 #3\else #2\fi
  }
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
\newcommand*\widebar[1]{\@ifnextchar^{{\wide@bar{#1}{0}}}{\wide@bar{#1}{1}}}
\renewcommand*\underbar[1]{\@ifnextchar_{{\under@bar{#1}{0}}}{\under@bar{#1}{1}}}
\newcommand*\wide@bar[2]{\if@single{#1}{\wide@bar@{#1}{#2}{1}}{\wide@bar@{#1}{#2}{2}}}
\newcommand*\under@bar[2]{\if@single{#1}{\under@bar@{#1}{#2}{1}}{\under@bar@{#1}{#2}{2}}}
\newcommand*\wide@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
    \let\mathaccent\save@mathaccent
    \if#32 \let\macc@nucleus\first@char \fi
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
    \ifdim\dimen@>\z@ \dimen@0pt\fi
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \overline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \overline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}
\newcommand*\under@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
    \let\mathaccent\save@mathaccent
    \if#32 \let\macc@nucleus\first@char \fi
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
    \ifdim\dimen@>\z@ \dimen@0pt\fi
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \underline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \underline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}
\makeatother


